Low-energy spectrum of Toeplitz operators: the case of wells

In the 1980s, Helffer and Sj\"ostrand examined in a series of articles the concentration of the ground state of a Schr\"odinger operator in the semiclassical limit. In a similar spirit, and using the asymptotics for the Szeg\"o kernel, we show a theorem about the localization properties of the ground state of a Toeplitz operator, when the minimal set of the symbol is a finite set of non-degenerate critical points. Under the same condition on the symbol, for any integer K we describe the first K eigenvalues of the operator.

==> Szego_projector_v2.tex <==
%Let $L^*$ denote the dual bundle of $L$, with $h^*$ the dual
%metric. It is itself a Riemannian manifold. Define
%\begin{align*}
%D&=\{(m,v)\in L^*,\, h^*(v)<1\}\\X&=\partial D = \{(m,v)\in L^*,\,
%h^*(v)=1\}.\end{align*}
%
%Then $X$ is a circle bundle on $M$, with a $S^1$-action on the fibres
%$r_{\theta}:(m,v)\mapsto (m,e^{i\theta}v)$. We will also denote by
%$\pi$ the projection from $X$ onto $M$.
%
%As $X$ is a submanifold of a Riemannian manifold, it inherits a
%volume form. Since $(L,h)$ is a prequantum bundle, $D$ is
%pseudoconvex, and the volume form on $X$ coincides with the Levi form.
%
%Let us consider the \emph{Hardy space} on $X$, defined as follows. 
%\begin{defn}
%\label{defn:Hardy-Szego}
%	We call \emph{Hardy space} on $X$ and denote by $H(X)$ the closed subspace of $L^2(X)$ consisting of functions which are
%	boundary values of holomorphic functions inside $D$.
%	The orthogonal projector from $L^2(X)$ onto $H(X)$ is denoted by $S$,
%	the \emph{Szeg\H{o}} projector.
%\end{defn}
%
%The scalar product on
%$L^2(X)$ is related to the one on $L^2(M)$ via the $\S^1$ action
%. If $x_0$ denotes any
%smooth section of $X$, one has, for any $u,v\in L^2(X)$:
%$$\langle u,v\rangle = \iint \overline{u}(r_{\theta}x_0(m))v(r_{\theta}x_0(m))
%\dd \theta \dd m.$$
%
%Using the $\S^1$ action, the space $H(X)$ can be further decomposed.
%For $N\in
%\N$, we can say
%that an element $f$ of $H$ is $N$-equivariant when, for each $x\in X$ and
%$\theta\in S^1$, the identity $f(r_{\theta}x)=e^{iN\theta}f(x)$
%holds. The space of $N$-equivariant functions is denoted by $H_N(X)$; then $H(X)$
%is the orthogonal sum of the different spaces $H_N(X)$ for $N\geq 1$. We will call
%$S_N$ the orthogonal projection on $H_N(X)$. Then the Schwartz kernel
%of $S_N$ is itself $N$-equivariant, in the sense that $$S_N(r_{\theta}x,r_{\phi}y)=e^{iN(\theta-\phi)}S_N(x,y).$$

